Regularizing Self-training for Unsupervised Domain Adaptation via Structural Constraints

Self-training based on pseudo-labels has emerged as a dominant approach for addressing conditional distribution shifts in unsupervised domain adaptation (UDA) for semantic segmentation problems. A notable drawback, however, is that this family of approaches is susceptible to erroneous pseudo labels that arise from confirmation biases in the source domain and that manifest as nuisance factors in the target domain. A possible source for this mismatch is the reliance on only photometric cues provided by RGB image inputs, which may ultimately lead to sub-optimal adaptation. To mitigate the effect of mismatched pseudo-labels, we propose to incorporate structural cues from auxiliary modalities, such as depth, to regularise conventional self-training objectives. Specifically, we introduce a contrastive pixel-level objectness constraint that pulls the pixel representations within a region of an object instance closer, while pushing those from different object categories apart. To obtain object regions consistent with the true underlying object, we extract information from both depth maps and RGB-images in the form of multimodal clustering. Crucially, the objectness constraint is agnostic to the ground-truth semantic labels and, hence, appropriate for unsupervised domain adaptation. In this work, we show that our regularizer significantly improves top performing self-training methods (by up to $2$ points) in various UDA benchmarks for semantic segmentation. We include all code in the supplementary.

==> sections/problem.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=\linewidth]{latex/figures/pipeline.png}
\caption{\textbf{Objectness Constraint Formulation:} Overall pipeline for computing the objectness constraint using multi-modal object-region estimates derived from RGB-Image and Depth-Map. Depth segmentation is obtained by clustering the histogram of depth values and  RGB segmentation is obtained via k-means clustering (SLIC) of raw-pixel intensities.  
Fusing these two types of segmentation yields object regions that are more consistent with the actual object. For example, a portion of the car in the middle is wrongly clustered with the road in depth segmentation and with the left-wall under RGB segmentation. However, the fused segmentation yields car-regions that completely respect the boundary of the car.} 
\label{fig:pipeline}
\end{figure*}

% \vspace{-0.15cm}
\section{Preliminaries}
%\section{Adaptation Via Self-Training }
\label{sec:problem_formulation}
We begin by introducing preliminary concepts on self-training based adaptation. These concepts serve as bases for introducing our objectness constraint in Section \ref{sec:approach} that is used to regularise the self-training methods. We refer to our framework as \texttt{PAC-UDA} which uses \textbf{P}seudo-labels \textbf{A}nd objectness \textbf{C}onstraints for self-training in \textbf{U}nsupervised \textbf{D}omain \textbf{A}daptation for semantic segmentation. Although, we describe a canonical form of self-training for formalising our regularisation constraint, \texttt{PAC-UDA} should be seen as a general approach that can encompass various forms of self-training (as shown in experiments).

\para{Unsupervised Domain Adaptation (UDA) for Semantic Segmentation:} Consider a dataset $D^s = \{(x_i^s, y_i^s)\}_{i=1}^{N_s}$ of input-label pairs sampled from a source domain distribution, $P_{X\times Y}^s$. The input and labels share the same spatial dimensions, $H \times W$,  where each pixel of the label is assigned a class $c\in \{1, \ldots, C\}$ and is represented via a $C$ dimensional one-hot encoding. We also have a dataset $D^t = \{(x_i^t, y_i^t)\}_{i=1}^{N_t}$ sampled from a target distribution, $P_{X\times Y}^t$ where the corresponding labels, $\{y_i^t\}$ are \textit{unobserved} during training. Here, the target domain is separated from the source domain due to domain shift expressed as  $P_{X\times Y}^s \neq P_{X\times Y}^t$. Under such a shift, the goal of unsupervised domain adaptation is to leverage $D^s$ and $D^t$ to learn a parametric model that performs well in the target domain. The model is defined as a composition of an encoder, $E_\phi:X \to \mathcal{Z}$ and a classifier, $G_\psi: \mathcal{Z} \to \mathcal{Z}_P $ where, $\mathcal{Z}\in \mathbb{R}^{H \times W \times d}$ represents the space of  $d$-dimensional spatial embeddings, $\mathcal{Z}_P\in \mathbb{R}^{H \times W \times C}$ gives the un-normalized distribution over the $C$ classes at each spatial location, and $\{\phi, \psi\}$ are the model parameters. To learn a suitable target model, the parameters are  optimised using a cross-entropy objective on the source domain, 
\begin{align}
L_\text{cls}^s &= -\frac{1}{N_s}\sum\limits_{i=1}^{N_s}\sum\limits_{m=1}^{H\times W}\sum\limits_{c=1}^{C}y_{imc}^s\log p^s_{imc}(\psi, \phi) \\
p^s_{imc}(\psi, \phi)  &= \sigma \left(G_\psi \circ E_\phi(x_i^s)\right)|_{m,c}~,
\label{eq:CEsrc}
\end{align}
\noindent where $\sigma$ denotes softmax operation and an adaptation objective over the target domain as described next.
 
\para{Pseudo-label self-training (PLST):} Following prior works \cite{zou2018unsupervised, Zhang2019CategoryAU}, we describe a simple and effective approach to PLST that leverages a source trained seed model to \textit{pseudo}-label unlabelled target data, via confidence thresholding.
% Continued training on the source data augmented with the pseudo labelled target data ultimately yields a model with superior performance on the target domain compared to the pretrained source model. 
Specifically, the seed model is first trained on $D^s$ using \eq\ref{eq:CEsrc} to obtain a good parameter initialisation, $\{\phi_0, \psi_0\}$. Then, this model is used to compute pixel-wise class probabilities, $p^t_{im}(\psi_0, \phi_0)$  using to \eq\ref{eq:CEsrc} for each target image, $x_i^t \in D^t$. These probabilities are used in conjunction with a predefined threshold $\delta$, to obtain one-hot encoded pseudo-labels
\begin{equation}
\tilde{y}_{imc}^t = 
\begin{cases}
1 ~\text{if}~ c=\arg\max\limits_{c'} p^t_{imc'} ~\text{and}~ p^t_{imc} \geq \delta\\
0 ~\text{otherwise} 
\end{cases} 
\label{eq:pslab}
\end{equation} 
Note that while \eq \ref{eq:pslab} uses a class-agnostic fixed 
threshold in practice, this threshold can be made class-specific and dynamically updated over the course of self-training.
Such a threshold ensures that only the highly-confident predictions contribute to successive training. The final self-training objective can be written in terms of pseudo-labels as  
\begin{equation}
L_\text{st}^t = -\frac{1}{N_t}\sum\limits_{i=1}^{N_t}\sum\limits_{m=1}^{H\times W}\sum\limits_{c'=1}^{C}\tilde{y}_{imc'}^t\log \left(p^t_{imc'}\right)
\label{eq:st}
\end{equation}
The overall UDA objective is simply, $L_\text{uda} = L_\text{cls}^s + \alpha_\text{st}  L_\text{st}^t$, where $\alpha_\text{st}$ is the relative weighting coefficients. 

==> temp.tex <==
something2
